A Combinatorial Approach to Neural Emergent Communication

Substantial research on deep learning-based emergent communication uses the referential game framework, specifically the Lewis signaling game, however we argue that successful communication in this game typically only need one or two symbols for target image classification because of a sampling pitfall in the training data. To address this issue, we provide a theoretical analysis and introduce a combinatorial algorithm SolveMinSym (SMS) to solve the symbolic complexity for classification, which is the minimum number of symbols in the message for successful communication. We use the SMS algorithm to create datasets with different symbolic complexity to empirically show that data with higher symbolic complexity increases the number of effective symbols in the emergent language.

==> sections/origin_of_language.tex <==
\section{The Origin of Language}
\label{sec:origin}
In exploring the genesis of language, two principal theories are often highlighted: continuity theories and discontinuity theories. Continuity theories posit that language is the culmination of a gradual evolutionary process, emerging from precursors and evolving incrementally rather than abruptly \cite{ulbaek1998origin}. For example, one of the scholars who support continuity theory, Bickerton contends that cognitive systems predate the emergence of language \cite{bickerton1990language}. Conversely, discontinuity theories argue that language emerged suddenly and intermediate stages cannot be bridged \cite{chomsky2006language}. This debate extends to the roots of language, with some scholars proposing that language evolved from communication, while others contend it originated from cognition. A notable example is Noam Chomsky, who has critiqued the relevance of animal communication studies in elucidating the evolution of human language. Chomsky further challenges the conventional view of language as primarily a means of conveying information, suggesting that human use of language is not characteristically informative in fact or in intention, therefore in some instances, can be misleading \cite{chomsky2006language}.

Hauser and colleagues emphasize the necessity of extensive interdisciplinary collaboration to comprehensively understand the faculty of language \cite{hauser2002faculty}. This faculty, in its broad sense (FLB), encompasses a sensory-motor system, a conceptual-intentional system, and, in its narrow sense (FLN), an internal computational system dedicated to managing recursion. A variety of empirical methodologies are employed to explore the evolution of these language faculties. For the sensory-motor system in the FLB, research includes vocal imitation and invention \cite{doupe1999birdsong}, neurophysiology of action-perception systems \cite{rizzolatti1998language}. For the conceptual-intentional system in the FLB, research includes theory of mind \cite{hare2000chimpanzees}, nonlinguistic conceptual representations \cite{cheney2018monkeys}, etc. For FLN, investigations include rule learning \cite{hauser2002retracted} and number representation \cite{matsuzawa1985use}. These comparative studies are pivotal for understanding the evolutionary processes and mechanisms underlying language faculties.

From the inception of artificial intelligence, a central endeavor has been to enable machines to emulate human cognitive processes \cite{turing2009computing}. Consequently, it is imperative to explore the parallels between language emergence in artificial intelligence and the evolution of the language faculty in both animals and humans. Such an exploration may yield valuable insights into the underlying reasons for the success or failure of computational methods. The subsequent sections of this paper will establish connections between computational methodologies and relevant literature in linguistics, psychology, and other related disciplines.
